Optimization for Robustness Evaluation beyond $\ell_p$ Metrics

Empirical evaluation of deep learning models against adversarial attacks entails solving nontrivial constrained optimization problems. Popular algorithms for solving these constrained problems rely on projected gradient descent (PGD) and require careful tuning of multiple hyperparameters. Moreover, PGD can only handle $\ell_1$, $\ell_2$, and $\ell_\infty$ attack models due to the use of analytical projectors. In this paper, we introduce a novel algorithmic framework that blends a general-purpose constrained-optimization solver PyGRANSO, With Constraint-Folding (PWCF), to add reliability and generality to robustness evaluation. PWCF 1) finds good-quality solutions without the need of delicate hyperparameter tuning, and 2) can handle general attack models, e.g., general $\ell_p$ ($p \geq 0$) and perceptual attacks, which are inaccessible to PGD-based algorithms.

==> Sections/section_elements/Fig-APGD-Obj-Pattern.tex <==
\begin{figure*}[!htbp]
\centering
\begingroup 
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{ccccc}
\centering
\small{AGPD-$\ell_1$-CE} 
&\small{AGPD-$\ell_1$-M} 
&\small{\pygranso-$\ell_1$-M}
&\small{APGD-$\ell_2$-CE}
&\small{APGD-$\ell_\infty$-CE}
\\
\includegraphics[width=0.12\linewidth]{Figures/APGD-Pattern/Err-Images/APGD-L1-CE-1000.png}
&\includegraphics[width=0.12\linewidth]{Figures/APGD-Pattern/Err-Images/APGD-L1-Margin-1000.png}
&\includegraphics[width=0.12\linewidth]{Figures/APGD-Pattern/Err-Images/PyGranso-L1-Margin-1000.png}
&\includegraphics[width=0.12\linewidth]{Figures/APGD-Pattern/Err-Images/APGD-L2-Margin-47.png}
&\includegraphics[width=0.12\linewidth]{Figures/APGD-Pattern/Err-Images/APGD-Linf-Margin-003.png}
\\
\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/HistoGrams/APGD-L1-CE-1000.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/HistoGrams/APGD-L1-Margin-1000.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/HistoGrams/PyGranso-L1-Margin-1000.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/HistoGrams/APGD-L2-Margin-47.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/HistoGrams/APGD-Linf-Margin-003.png}
\\
\hline 
\vspace{-4pt}
\\
\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/Sparsity-HistoGram/APGD-L1.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/Sparsity-HistoGram/APGD-Margin-L1.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/Sparsity-HistoGram/PyGranso-Margin-L1.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/Sparsity-HistoGram/APGD-L2.png}
&\includegraphics[width=0.16\linewidth]{Figures/APGD-Pattern/Sparsity-HistoGram/APGD-Linf.png}
\end{tabular}
\endgroup 
\caption{Sparsity patterns of the perturbations found by different algorithm-distance-loss combinations when attacking the \texttt{pat\_alexnet\_0.5} model~\cite{laidlaw2021perceptual} using \cref{eq:robust_loss}. \textbf{1st row}: different perturbations $\mb \delta$'s on a fish image; \textbf{2nd row}: histograms of pixels inside each perturbation $\mb \delta$; \textbf{3rd row}: histograms of the sparsity measure $\norm{\mb \delta}_1/\norm{\mb \delta}_2$ over $1024$ images randomly selected from ImageNet100. Here, CE: cross-entropy loss; M: margin loss, and we set $\eps=1000$ for all $\ell_1$ attacks, $\eps = 4.6$ for all $\ell_2$, and $\eps = 0.03$ for all $\ell_\infty$, respectively. } 
\label{Fig:APGD Patterns}
\end{figure*}

==> Sections/section_elements/Fig-APGD-Pattern.tex <==
\begin{figure}
\centering
\begin{tabular}{ccc}
\centering
\includegraphics[width=0.22\linewidth]{Figures/APGD-Norm-Pattern/APGD-CE-L1-Pattern.png} &
\includegraphics[width=0.22\linewidth]{Figures/APGD-Pattern/L2-Err.png} &
\includegraphics[width=0.22\linewidth]{Figures/APGD-Pattern/Linf-Err.png}\\
\centering
\small{(a) $\delta$~ - ~$l_{1}$} 
& \small{(b) $\delta$~ - ~$l_{2}$ }
& \small{(c) $\delta$~ - ~$l_{\infty}$} \\
\centering
\includegraphics[width=0.3\linewidth]{Figures/APGD-Norm-Pattern/APGD-CE-L1-Histo.png} &
\includegraphics[width=0.3\linewidth]{Figures/APGD-Pattern/L2-Histo.png} &
\includegraphics[width=0.3\linewidth]{Figures/APGD-Pattern/Linf-Histo.png}\\
\centering
\small{(d) $\delta$ histogram~ - ~$l_{1}$} 
& \small{(e) $\delta$ histogram~ - ~$l_{2}$ }
& \small{(f) $\delta$ histogram~ - ~$l_{\infty}$} \\
  
\end{tabular}
\caption{Visualization of the solution patterns using APGD attacks.}

\label{Fig: APGD Solution Patterns}
\end{figure}

==> Sections/section_elements/Fig-Min-Patter.tex <==
\begin{figure*}[!htbp]
\centering
\begingroup 
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabular}{ccc}
\centering
\small{FAB-$\ell_1$} 
&\small{FAB-$\ell_2$} 
&\small{FAB-$\ell_\infty$}
\\
\includegraphics[width=0.3\linewidth]{Figures/FAB-Pattern/Err-Images/L1-Err.png}
&\includegraphics[width=0.3\linewidth]{Figures/FAB-Pattern/Err-Images/L2-Err.png}
&\includegraphics[width=0.3\linewidth]{Figures/FAB-Pattern/Err-Images/Linf-Err.png}
\\
\includegraphics[width=0.3\linewidth]{Figures/FAB-Pattern/HistoGrams/L1-histo.png}
&\includegraphics[width=0.3\linewidth]{Figures/FAB-Pattern/HistoGrams/L2-histo.png}
&\includegraphics[width=0.3\linewidth]{Figures/FAB-Pattern/HistoGrams/Linf-histo.png}
\\
\hline 
\vspace{-4pt}
\\
\includegraphics[width=0.16\linewidth]{Figures/FAB-Pattern/Sparsity-HistoGram/adv_image_0.png}
&\includegraphics[width=0.16\linewidth]{Figures/FAB-Pattern/Sparsity-HistoGram/adv_image_0.png}
&\includegraphics[width=0.16\linewidth]{Figures/FAB-Pattern/Sparsity-HistoGram/adv_image_0.png}
\end{tabular}
\endgroup 
\caption{Sparsity patterns of the perturbations found by FAB when attacking the \texttt{pat\_alexnet\_0.5} model~\cite{laidlaw2021perceptual} using \cref{eq:robust_loss}. \textbf{1st row}: different perturbations $\mb \delta$'s on a fish image; \textbf{2nd row}: histograms of pixels inside each perturbation $\mb \delta$; \textbf{3rd row}: histograms of the sparsity measure $\norm{\mb \delta}_1/\norm{\mb \delta}_2$ over $1024$ images randomly selected from ImageNet100. } 
\label{Fig:APGD Patterns}
\end{figure*}

==> Sections/section_elements/Table-Pattern-Compare.tex <==
\begin{table*}[!htpb]
\caption{Quantification of the complementarity of different attack methods. Each base (each column) is augmented with \textbf{Att. 1} and \textbf{Att. 2} to form two variants that only differ by a single factor; APGD is the default when no method is declared. Each model we attack is always adversarially-trained by variant $1$, and then we attack the trained model using both variants. The last column is on ImageNet100, and all other columns are on CIFAR10. For each column, over the union of attack successes by both variants, we calculate the percentage of \textbf{intersection}, and those attacked only by one of the variants, i.e., the \textbf{Only Att. 1} and \textbf{Only Att. 2} rows. (iter: \#iterations in APGD; dense init: initialize with $\mb x_0 + 0.2\cdot \mb 1$; LPIPS-$\ell_{p}$: using $\ell_{p}$ norm for the distance calculation in \cref{Eq. LPIPS Constraint}).
% The union of attack success by both methods is set to be $100 \%$. Table below shows the distribution of the attack success of a given pair of attack, where 1) \textbf{intersection} is the attack success achieved by both attacks; 2) \textbf{Only Att. 1} and \textbf{Only Att. 2} are the attack success only achieved by a single attack. Here, CE: cross-entropy loss; M: margin loss; $l_{\cdit}$: norm constraint; iter---number of iterations in APGD; Dense Init: intialize with $x_0 + 0.2\mb 1$; LPIPS-$l_{p}$: using $l_{p}$ norm to represent $d(\mb x, \mb x')$ in \cref{Eq. LPIPS Constraint}. } \textcolor{red}{The LPA-M ($l_1 = 500$) solution mostly lie in the $l_2 = 0.5$ ball in the LPIPS space.
}
\label{tab: pattern comare}
\begin{center}
\setlength{\tabcolsep}{1.0mm}{
%\renewcommand\arraystretch{1.25}
\begin{tabular}{l | c c c c c c c c |c}

\small{\textbf{Base}}
&{}
&\small{$\ell_1$-M}
&\small{$\ell_1$-M}
&\small{$\ell_1$}
&\small{$\ell_1$-M}
&\small{$\ell_2$-M}
% &\small{APGD-$l_1$-M}
% &\small{APGD-$l_1$-M}
&\small{M}
&\small{M}
&\small{LPA-M}
\\
\toprule
\small{\textbf{Att. 1}}
&{}
&\small{$\mb x_0$ init.}
&\small{$100$ iter.}
&\small{M}
&\small{}
&\small{}
% &\small{$x_0$ Init.}
% &\small{100 iter.}
&\small{$\ell_2$}
&\small{$\ell_2$}
&\small{LPIPS-$\ell_2$}
\\
\midrule
\small{\textbf{Att. 2}}
&{}
&\small{dense init.}
&\small{10 iter.}
&\small{CE}
&\small{PWCF}
&\small{PWCF}
% &\small{Dense Init.}
% &\small{10 iter.}
&\small{PWCF-$\ell_4$}
&\small{$\ell_1$}
&\small{LPIPS-$\ell_1$}
\\
\midrule
\small{\textbf{Intersection (\%)}}
&{}
&{$96.5$}
&{$81.3$}
&{$91.7$}
&{$43.3$}
&{$37.3$}
% &{$96.5$}
% &{$81.3$}
&{$50.6$}
&{$43.3$}
&{$60.0$}
\\
\midrule
\small{\textbf{Only Att. 1 (\%)}}
&{}
&{$2.93$}
&{$18.7$}
&{$5.89$}
&{$56.7$}
&{$0.03$}
% &{$2.93$}
% &{$18.7$}
&{$34.1$}
&{$0.9$}
&{$0$}
\\
\midrule
\small{\textbf{Only Att. 2 (\%)}}
&{}
&{$0.57$}
&{$0.02$}
&{$3.44$}
&{$0.00$}
&{$62.6$}
% &{$0.57$}
% &{$0.02$}
&{$15.2$}
&{$55.8$}
&{$40.0$}
\\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}
